Machine Learning and Statistical Insights into Hospital Stay Durations: The Italian EHR Case

Length of hospital stay is a critical metric for assessing healthcare quality and optimizing hospital resource management. This study aims to identify factors influencing LoS within the Italian healthcare context, using a dataset of hospitalization records from over 60 healthcare facilities in the Piedmont region, spanning from 2020 to 2023. We explored a variety of features, including patient characteristics, comorbidities, admission details, and hospital-specific factors. Significant correlations were found between LoS and features such as age group, comorbidity score, admission type, and the month of admission. Machine learning models, specifically CatBoost and Random Forest, were used to predict LoS. The highest R2 score, 0.49, was achieved with CatBoost, demonstrating good predictive performance.

==> sections/01-introduction.tex <==
\section{Introduction}
\label{sec:introduction}
\vspace{\secVspaceAfter}

Length of stay (LoS) is an important indicator of the use of medical services that is used to assess the efficiency of hospital management, patient quality of care, and functional performance~\cite{Gokhale2023}. Shorter LoS has been associated with decreased risks of infections, improvements in treatment outcomes, reduced medical costs, and increased hospital bed turnover~\cite{Bueno2010,Rotter2010}.

LoS among patients with the same condition or undergoing the same type of intervention can vary due to complex factors related to the individual patient characteristics, differences in medical processes and practices across facilities~\cite{Baek2018}, and external influences such as seasonal trends and public health crises. Hence, in order to understand which factors are associated with LoS, these factors should be taken into account.

% In this study, electronic health records (EHR) data and machine learning techniques were used to analyze patient hospitalization logs from over 60 Italian healthcare facilities registered over a four-year period. 
In this study, electronic health records (EHR) data from the TrustAlert research project\footnote{https://www.trustalert.it/}, an Italian initiative aimed at developing early warning, monitoring, and forecasting tools for public health agencies, were used to analyze patient hospitalization logs from over 60 Italian healthcare facilities over a four-year period.
This allowed us to examine multiple factors influencing LoS. 
The aim of this study was to provide practical insights that could help hospitals manage the duration of inpatient stays more efficiently.

The remainder of the paper is structured as follows. The Methodology section (Section~\ref{sec:methodology}) describes the main data characteristics (Section~\ref{sec:data}), followed by details regarding predictive features for length of stay (Section~\ref{sec:predictive-features}). We then outline the approach for statistical analysis (Section~\ref{sec:statistical-analysis}), aimed as examining the relationship between features and length of stay, as well as predictive modeling and evaluation (Section~\ref{sec:predictive-modeling}). The Results section (Section~\ref{sec:results}) presents findings from the statistical analysis (Section~\ref{sec:statistical-analysis-results}) and machine learning models (Section~\ref{sec:prediction-results}). Finally, Section~\ref{sec:conclusions} provides conclusions and directions for future work.

==> sections/03-methodology.tex <==
\section{Methodology}
\label{sec:methodology}
\vspace{\secVspaceAfter}

% \subsection{Data and Preprocessing}
\subsection{Data}
\label{sec:data}
\vspace{\secVspaceAfter}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figs/los_distribution_combined.pdf}
\vspace{-.5cm}
\caption{Distribution of length of stay in days overall (left) and for specific years (right). In the violin plots, observations above the 98th percentile have been excluded for clarity, while horizontal bars denote the 25th, 50th (median), and 75th percentiles.}
\label{fig:los-distribution}
\vspace{\figVspaceAfter}
\end{figure}

Inpatient hospitalization records between January 2020 and December 2023 were extracted from the EHRs of 66 healthcare facilities, spanning 52 departments, in Piedmont, Italy, to analyze factors correlating with the length of hospital stay. Table~\ref{tab:data_description} provides an overview of the data set characteristics, while Table~\ref{tab:healthcare_facilities} presents the various categories of these facilities. 
For the full four-year period (2020-2023), we selected 59,684 hospitalization records of one day or longer involving 37,526 distinct patients. For each record, both admission and discharge date were available, which allowed the calculation of the length of stay. Each record included a de-identified (hashed) patient identifier, enabling the reconstruction of hospitalization histories. Additionally, each record included age group, hospitalization type, diagnosis, and intervention. Records were categorized into three types of admissions: day hospital medical treatments, day hospital surgical procedures, or standard inpatient admissions. While day hospital treatments are typically intended for short stays, some cases extended beyond one day, likely due to the complexity of the treatment. Diagnoses and interventions were coded according to the 9th revision of the International Classification of Diseases (ICD-9), including the ICD-9 Procedure Coding System (PCS). 
% TBD: procedures

\begin{table}[t]
    \centering
    \caption{Summary of data set characteristics (example data is artificial).}
    \label{tab:data_description}
    \smallskip
    \footnotesize
    \renewcommand{\arraystretch}{\tabArrayStretch}
    \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{3cm} *{2}{>{\raggedright\arraybackslash}X}}
        \toprule
        \textbf{Variable} & \textbf{Value} & \textbf{Example} \\
        \midrule
        Hashed patient ID & 37,526 unique patients & JL(\&LFURP(!2 \\
        Age group & 20 categories & 35-39\\ 
        Diagnosis code & 3,689 ICD-9 unique codes & 724.2 - Lumbago\\ 
        Procedure code & 1,645 ICD-9 unique codes & 88.93 - MRI of the Spinal Canal \\
        Facility & 66 unique values & Az. Ospedal. S. Croce E Carle \\
        Department & 52 unique values & Neurology \\
        Hospitalization type & Surgical, medical, ordinary & Medical \\
        Admission date & 01/01/2020 – 31/12/2023 & 22/07/2021 \\  
        Discharge date & 01/01/2020 – 31/12/2023 & 25/07/2021 \\       
        \bottomrule
    \end{tabularx}	
    \vspace{\tabVspaceAfter}
\end{table}

\begin{table}[h]
    \centering
    \caption{Counts of healthcare facilities per category.}
    \label{tab:healthcare_facilities}
    \smallskip
    \footnotesize
    \renewcommand{\arraystretch}{\tabArrayStretch}
    \begin{tabularx}{\textwidth}{Xrrr}
        \toprule
        \textbf{Category} & \textbf{Count} & \textbf{Sample count} & \textbf{\% samples} \\
        \midrule
        General and teaching hospitals                  & 13 & 9,806  & 16.43  \\
        Specialized hospitals                           & 6  & 3,449  & 5.78   \\
        Private clinics and rehabilitation centers      & 21 & 7,985  & 13.38  \\
        Local and community hospitals                   & 19 & 37,344 & 62.57  \\
        Geriatric and long-term care facilities         & 2  & 391    & 0.66   \\
        Religious or charitable medical facilities      & 2  & 555    & 0.93   \\
        Rehabilitation centers and research institutes  & 3  & 154    & 0.26   \\[2.5pt]
        \textit{Total} & \textit{66} & \textit{59,684} & \textit{100.00} \\
        \bottomrule
    \end{tabularx}
    \vspace{\tabVspaceAfter}
\end{table}


Figure~\ref{fig:los-distribution} illustrates the distribution of the length of stay. The right panel shows the distribution of the length of stay separately for each year. 
% The violin plots include samples up to the 98th percentile for better clarity. 
In terms of hospitalization share, 2020 accounts for 17\% of sample, while 2021, 2022, and 2023 contribute approximately 25\%, 28\% and 30\% percent, respectively. 
% The width of each violin plot at a given y-axis value represents the density of hospital stays of that duration, while horizontal bars indicate the 25th, 50th (median), and 75th percentiles. 
Table~\ref{tab:los_statistics} shows key statistics for each year. Notably, for each following year, the plot shows broader section around the median, meaning higher concentration around the typical values. In contrast, the years 2020 and 2021 exhibit larger interquartile ranges (IQRs) compared to 2022 and 2023, suggesting greater variability and unpredictability in the length of stay during those earlier years.
These patterns likely reflect the influence of the COVID-19 pandemic. In 2020 and 2021, hospitals experienced severe strain with a mix of short and prolonged hospitalizations, while 2022 and 2023 show more consistent hospitalization patterns.


\begin{table}[t]
    \centering
    \caption{Yearly statistics for the length of hospital stay.}
    \label{tab:los_statistics}
    \smallskip
    \footnotesize
    \renewcommand{\arraystretch}{\tabArrayStretch}
    \begin{tabularx}{\textwidth}{*{8}{>{\Centering}X}}
        \toprule
        \textbf{Year} & \textbf{Number} & \textbf{\%} & \textbf{Median} & \textbf{Std} & \textbf{IQR} & \textbf{Min} & \textbf{Max} \\
        \midrule
        2020 & 10147 & 17.00 & 5.0  & 20.80 & 2-11 & 1  & 362 \\
        2021 & 15142 & 25.37 & 5.0  & 23.67 & 2-11 & 1  & 360 \\
        2022 & 16674 & 27.94 & 4.0  & 22.74 & 2-10 & 1  & 357 \\
        2023 & 17721 & 29.69 & 4.0  & 16.17 & 2-9  & 1  & 328 \\
        \bottomrule
    \end{tabularx}
    \vspace{\tabVspaceAfter}
\end{table}


\subsection{Features}
\label{sec:predictive-features}
\vspace{\secVspaceAfter}

In this study, we examine a set of features that can be broadly classified into three categories: patient-related, admission-related, and hospital-related characteristics. An overview of these features is provided in Table~\ref{tab:variables-description}. These feature categories have been explored in previous studies on length of stay prediction (see~\cite{Gokhale2023} and references therein). In this study, we present a systematic analysis of these features and their relationship with LoS, using a dataset of novel hospitalizations in Piedmont. % , with consideration of data availability limitations

We started with the raw hospitalization dataset and transformed it into a structured feature dataset. For each entry in the original dataset, a corresponding record was created in the feature dataset. In some cases, the data were used directly, while in others, we applied transformations that incorporated historical records, as detailed below. 
This feature set was then analyzed for its relationship with length of stay (LoS) across all hospitalizations, using both statistical and predictive methods, as detailed in the following sections.

\begin{table}[t]
    \centering
    % \caption{Description of variables used in the analysis.}
    \caption{Description of features used in the analysis.} % , categorized into patient, admission, and hospital characteristics.
    \label{tab:variables-description}
    \smallskip
    \footnotesize
    \renewcommand{\arraystretch}{\tabArrayStretch}
    \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{2.6cm} >{\raggedright\arraybackslash}X}
        \toprule
        \textbf{Variable} & \textbf{Description} \\ 
        \midrule
        Age group & Age category as a four-year interval (e.g., 0 for newborns, 1-4, up to 90+). \\
        \# of comorbidities & Count of unique comorbid conditions based on past diagnoses. \\
        Comorbidity index & Elixhauser comorbidity index. \\
        Diagnosis & Diagnosis associated with the hospitalization. \\
        Procedure & Medical procedure performed during hospitalization. \\
        Admission type & Hospitalization type: day hospital (medical/surgical) or standard inpatient. \\
        Admission month & Month when the hospitalization occurred. \\
        Patient volume & Adjusted hospitalizations for a diagnosis in the past three months. \\
        Historical LoS & Average LoS for a diagnosis and hospital over the past three months. \\
        \bottomrule
    \end{tabularx}
    \vspace{\tabVspaceAfter}
\end{table}


\vspace{\parVspaceBefore}
\paragraph{Patient characteristics.}
The patient's age group is taken directly from the hospitalization record and is represented as a categorical variable based on four-year intervals, starting with \emph{0} (newborns), followed by \textit{1–4}, \textit{5–9}, and so on, up to \textit{90+}. 
%
We computed the number of comorbidities and the Elixhauser comorbidity index~\cite{Elixhauser1998}, which quantify a patient's overall health, and have been previously associated with LoS~\cite{Liu2019}.
These calculations were based on the patient's disease history, which we constructed by extracting unique ICD-9 codes for prior diagnoses of a patient using admission dates to establish time ordering.
We leveraged Python's comorbidity (\texttt{comorbiPy}) library\footnote{\url{https://comorbidipy.readthedocs.io/en/latest/}.} to calculate comorbidity measures.

\vspace{\parVspaceBefore}
\paragraph{Admission characteristics.}
We experimented with both embedding-based and categorical representations for diagnoses and procedures. In the categorical approach, ICD-9 codes were encoded as discrete variables, while in the embedding-based approach, numerical vectors represented semantic relationships.
%
For diagnoses, we employed previously published 100-dimensional embeddings from Kane et al.~\cite{Kane2023}, which were originally designed for ICD-10 codes. 
These embeddings, derived from the BioGPT large language model (LLM)~\cite{Luo2022}, capture the hierarchical structure of ICD codes. 
To integrate these embeddings, we mapped ICD-9 codes to ICD-10 codes using the official \emph{General Equivalence Mappings} incorporated into Python's \texttt{icdmappings} library\footnote{\url{https://pypi.org/project/icd-mappings/}.}. 
%
For procedures, we employed a similar approach, using 300-dimensional embeddings developed by Choi et al.~\cite{Choi2016}, which were trained with a neural language model to capture similarities between procedures.
%
% Incorporating these embeddings into the predictive model reduces its complexity compared to using categorical values, as similar conditions share similar embeddings, and similar procedures also share their own distinct embeddings.
To account for seasonal trends and variations in admission types, we included both month of admission and type of admission as features, directly extracted from hospitalization records.

\vspace{\parVspaceBefore}
\paragraph{Hospital characteristics.}
We included the hospital patient volume feature, defined as the number of patients admitted with a specific diagnosis over the past three months, normalized by the actual number of observation days. Previous studies indicated that higher-volume hospitals may possess greater experience, specialized expertise, and more established care protocols~\cite{Kahn2006,Birkmeyer2002}. Given these factors, it is reasonable to hypothesize that hospital volume could influence length of stay.
% We included the hospital patient volume feature, which we defined as the number of patients admitted with a given diagnosis over the past three months. This computation was normalized to account for the actual number of observation days. Prior research suggests that higher-volume hospitals may have greater experience, specialized expertise, and well-developed care protocols~\cite{Kahn2006,Birkmeyer2002}. Given these factors, hospital volume may reasonably influence length of stay. 
%
To account for variations in LoS across hospitals, we introduced a feature that reflected the historical average hospitalization duration, considering the hospital, department, and specific diagnosis of the hospitalization record. 
The computation of this feature began by calculating the \emph{observed mean} of LoS for the given diagnosis in the same hospital and department. To cope with data scarcity for some combinations of diagnosis, hospital, and department (possibly leading to unreliable observed means), we also computed a \emph{global mean} that represents the average LoS for related diagnoses across previous hospitalizations at the same hospital. Related diagnoses were identified using the \texttt{drgpy} library\footnote{\url{https://github.com/yubin-park/drgpy}.}, which assigns diagnosis codes to Diagnosis Related Groups (MS-DRG)~\cite{DRGDesignDevelopment}. MS-DRG is a system used in the U.S. for inpatient reimbursement, grouping diagnoses that share similar hospital resource usage. A smoothed mean was then computed by combining the observed and global means, using a Bayesian smoothing approach~\cite{Sheetrit2019} with a smoothing parameter set to five.

\subsection{Statistical Analysis}
\label{sec:statistical-analysis}
\vspace{\secVspaceAfter}

The statistical analysis explored factors influencing LoS from multiple angles. A subset of features with less obvious influence on LoS was selected for this analysis. Specifically, we considered all features in Table~\ref{tab:variables-description} except diagnosis, procedure and historical LoS.
%
The number of comorbidities and comorbidity index were discretized into categories~\cite{Austin2015}, while other categorical variables (age group, admission type, and admission month) were used directly. The relationship between each of these variables and LoS was then assessed using the Kruskal-Wallis test~\cite{Carter2014}, which is robust to non-normal distributions and suitable for comparing LoS across independent groups. Additionally, LoS variability within each category was summarized by the median, interquartile range, and standard deviation.
%
For patient volume, we first calculated the number of patients and average LoS for each diagnosis-hospital pair. Using this aggregated data, a mixed-effects linear model was then fitted with average LoS as the outcome variable, patient volume as the independent variable, and diagnosis as a random effect. This approach accounts for diagnosis-specific variability and evaluates whether higher patient volume is associated with lower LoS.
%
Statistical significance was assessed at a 0.05 significance level to identify meaningful associations. The results are presented in Section~\ref{sec:statistical-analysis-results}.

\subsection{Predictive Modeling}
\label{sec:predictive-modeling}
\vspace{\secVspaceAfter}

\paragraph{Machine Learning Models.} We employed machine learning models to assess the predictive power of the considered features (see Table~\ref{tab:variables-description}). 
Due to likely complex, non-linear relationship between features and length of stay, we framed the task as a non-linear regression problem and employed two robust tree-based models: Random Forest and CatBoost~\cite{Prokhorenkova2018}.
Both models are known for effective handling large and diverse data sets, and previous studies have demonstrated that they outperform other regression models in predicting length of stay~\cite{Jain2024}. 
% Random Forest uses multiple decision trees to reduce overfitting and achieve model generalization. On the other hand, CatBoost is specifically optimized for categorical data and often outperforms other gradient boosting algorithms in structured data sets, particularly when dealing with large numbers of categorical features~\cite{Prokhorenkova2018}. f
% These models not only allowed us to address LoS prediction task but also provided insights into the relative importance of different features in determining hospitalization durations.
% \noindent
Interestingly, the models exhibited different sensitivities to how categorical features were represented. CatBoost performed best when diagnosis and procedure features were used as categorical variables, likely because of its built-in target encoding, which encodes each category based on the mean value of the target variable for that category. In contrast, Random Forest showed weaker performance when categorical features were used directly or one-hot encoded but performed best when represented as embeddings. 
In our results (Section~\ref{sec:prediction-results}, we present only the best-performing configurations: embeddings for Random Forest and categorical variables for CatBoost.

\vspace{\parVspaceBefore}
\paragraph{Validation Approach.} 
Given the seasonal trends exhibited by LoS, we split data into training, validation and test sets on a per-year basis to both enable and properly assess the capability of the model to capture potential seasonal variations in our data.
% We set the window size to a full year to enable the model to capture potential seasonal variations. 
To assess the impact of additional historical data on model performance, we designed two validation scenarios. In the first scenario, machine learning algorithms were trained on hospitalization records from 2021, validated on 2022 records, and tested on 2023 records. In the second scenario, a larger training data set was used, incorporating hospitalization records from both 2020 and 2021, followed by validation on 2022 records and testing on 2023 records. 
By comparing these two setups, we assessed whether including additional historical data improves model performance.

\vspace{\parVspaceBefore}
\paragraph{Evaluation.} To evaluate the quality of fit, we used adjusted R$^2$ and mean absolute error (MAE). We assessed these metrics for both the training and validation sets. Adjusted R$^2$ measures the proportion of variance explained by the model. Because it accounts for the number of predictors, it is more suitable than standard R$^2$ when comparing models with different feature sets~\cite{james2013introduction}. A consistently high adjusted R$^2$ value across the training and validation sets suggests that the model captures a significant portion of variability without overfitting. On the other side, MAE offers a straightforward measure of prediction accuracy by averaging the absolute differences between predicted and actual values. To evaluate the generalizability of the models on the test sets, in addition to MAE we used also root mean squared error (RMSE), which in contrast to MAE, penalizes large errors more heavily due to squaring~\cite{bishop2006pattern}.


% TO DISCUSS: possible settings to run experiments according to the intent of preserving the temporal aspects that we want to analyze
% \begin{itemize}
% \item to split the data set in batches preserving relevant temporal sequences. For example:
%     \begin{itemize}
%     \item adopting a sliding window approach in which 4 months are used for training and the subsequent fifth month for test;
%     \item to predict the value of a specific month (e.g., January), use the data of the last January for test and data of all the previous January for train;
%     \item ...
%     \end{itemize}
% \item to remove ``facility'' and ``department'' from the model by demonstrating the impact of geographical information;
% \item to select a few (e.g., 3) language models from the state of the art in order to compare their impact on the ICD 10 encoding of the content of diagnosis fields.
% \end{itemize}

% \noindent 
% \textbf{***} \newline
% Possible directions exploiting longitudinal aspect of the EHR data set, and inclusion of data from multiple hospitals:
% \begin{itemize}
%     \item Investigate hospital-specific variability. Approach: train models using aggregated hospital-level metrics, such as average LoS (by diagnosis, age\_group); compare these to models using the hospital variable. Evaluation approach: cross-validation across hospital groups.
%     \item Investigate how feature importance/predictive ability changes over time. Approaches:
%     \begin{itemize}
%         \item Incrementally increase the training set size by adding data from subsequent periods. 
%         \item Apply rolling-window validation, e.g., by using 1-year of window data. The shift size could be six months.
%     \end{itemize}     
% \end{itemize}
